Binding-Adaptive Diffusion Models for Structure-Based Drug Design

Structure-based drug design (SBDD) aims to generate 3D ligand molecules that bind to specific protein targets. Existing 3D deep generative models including diffusion models have shown great promise for SBDD. However, it is complex to capture the essential protein-ligand interactions exactly in 3D space for molecular generation. To address this problem, we propose a novel framework, namely Binding-Adaptive Diffusion Models (BindDM). In BindDM, we adaptively extract subcomplex, the essential part of binding sites responsible for protein-ligand interactions. Then the selected protein-ligand subcomplex is processed with SE(3)-equivariant neural networks, and transmitted back to each atom of the complex for augmenting the target-aware 3D molecule diffusion generation with binding interaction information. We iterate this hierarchical complex-subcomplex process with cross-hierarchy interaction node for adequately fusing global binding context between the complex and its corresponding subcomplex. Empirical studies on the CrossDocked2020 dataset show BindDM can generate molecules with more realistic 3D structures and higher binding affinities towards the protein targets, with up to -5.92 Avg. Vina Score, while maintaining proper molecular properties. Our code is available at https://github.com/YangLing0818/BindDM

==> sections/Rebuttal.tex <==
We thank all the reviewers for the valuable feedback. 
% Please see below for our responses to the comments.

\noindent\textbf{\textcolor{magenta}{--------------------- Response to Reviewer \#1 ------------------}}
% We thank the reviewer for the valuable feedback. Please see below for our responses to the comments. 

% \noindent{\textbf{\textcolor{blue}{Q1: Why is the training script not provided during the review process?}}} 
\noindent{\textbf{\textcolor{blue}{Q1: Why is the training script not provided?}}} 
% Because of organizational policy requirements, we are committed to open the source code of training and inference upon paper acceptance.
% Because of organizational policy requirements, we are committed to open the source code upon paper acceptance.
We are committed to open the source code upon paper acceptance.

\noindent\textbf{\textcolor{magenta}{--------------------- Response to Reviewer \#3 ------------------}}
% We thank the reviewer for the valuable feedback. Please see below for our responses to the comments. 

% \noindent{\textbf{\textcolor{blue}{Q1: Can the authors give an explanation on whether the hypothesis of given binding sites make the original problem of molecular generation less significant? Or putting it more correctly, does it make the problem more trivial?}}} 
% \noindent{\textbf{\textcolor{blue}{Q1: Can the authors give an explanation on whether the hypothesis of given binding sites make the problem more trivial?}}} 
\noindent{\textbf{\textcolor{blue}{Q1: Whether the hypothesis of given binding sites make the problem more trivial?}}} 
% By considering the given protein pockets during the generation process of molecular ligands, it requires the model to not only focus on generating geometrically and chemically plausible ligands but also take into account the additional geometric and chemical constraints imposed by the given protein pockets.
% The motivation behind our approach is to adaptively exploit binding-related information from the complex during the iterative molecule generation process. This is designed for enhancing the generation process, as complete complexes often contain a large number of atoms and redundant information is not related to the binding.
% Our experiments presented \textbf{\cref{tab:abla_component} (Exp0 and Exp1)} and \textbf{\cref{fig:subcomp_acc}} verified that our method is capable of \textbf{mining some binding-related information} from the original complex.
% The details of differences between our method and the existing diffuion-based method (TargetDiff and DecompDiff) please refer to the response to \textbf{the Q2 of Reviewer\#7}. 
% It is worth noting that our method \textbf{does not rely on additional ligand information as templates} for the generation process. 
% Unlike DecompDiff, which is a two-stage method requiring an open-source software to obtain the anchor atoms of ligands as templates, \textbf{our method performs the entire generation process from scratch}. 
% Compared with DecompDiff, our method is a single-stage method generates molecules from scratch. Therefore, our method has better generalization capabilities (for example, higher diversity metrics presented in \textbf{\cref{tab:main_tab}}.) and less framework complexity than DecompDiff.
% And DecompDiff is a \textbf{two-stage} method and \textbf{totally different} with ours. Specifically, it \textbf{relies on an open-source software, AlphaSpace}, to obtain anchors atoms of generated ligands as \textbf{templates} for the subsequent generation process, which not only \textbf{increases the complexity} of the framework but also \textbf{reduces the generalization ability} of the model, as present in Diversity and QED metrics of \textbf{\cref{tab:main_tab}}. 
% It worth noting that our method does not assume binding sites of protein pocket is known. The substructure extraction process in our method is adaptively learned during the iterative molecule generation process, and without using any external software for providing binding-related knowledge like DecompDiff. Compared with DecompDiff, our method is a single-stage method generates molecules from scratch. Therefore, our method has better generalization capabilities (for example, higher diversity metrics presented in \textbf{\cref{tab:main_tab}}.) and less framework complexity than DecompDiff.
It is worth noting that our method \textbf{does not} assume the binding sites within the protein pocket are given. The extraction of binding-related subcomplexes (potential binding sites) in our method is \textbf{adaptively learned} during the iterative molecule generation process, \textbf{without} relying on any external software or pre-existing binding knowledge. Unlike DecompDiff which relies on molecule-agnostic binding priors, our method is a \textbf{single-stage approach that generates molecules from scratch}, which has \textbf{better generalization capabilities} (with higher diversity presented in \textbf{\cref{tab:main_tab}}) and \textbf{simpler frameworks}. 
% The details of differences between our method and the existing diffuion-based method please refer to the response to \textbf{the Q2 of Reviewer\#7}. 

% \noindent{\textbf{\textcolor{blue}{Q2: In Figure 2, the notation of GTM is not found.}}} The GTM is defined in \cref{fig:GTM}, and we will provide the process of GTM in the form of formulas in the final version of paper.
% We directly illustrate the process of the gated transmission module (GTM) in \cref{fig:GTM}, since operations used in GTM are commonly known we do not give specific design details.
% We will provide the complete process of GTM in the form of formulas in the final version of the paper.


% \noindent{\textbf{\textcolor{blue}{Q3: A model that is dependent on the extracted binding sites seems to have less generalization capabilities, due to the requirement of the ligand structure information, in order to locate the pockets?}}}
% \noindent{\textbf{\textcolor{blue}{Q2: The model has less generalization capabilities, due to the requirement of the ligand structure information, in order to locate the pockets?}}}
% In our method, the generation of molecular ligands is performed entirely from scratch, without relying on any templates. Throughout the molecular generation process, we iteratively refine and extract binding-related subcomplexes from the original complexes. 
% This approach differs significantly from DecompDiff and our model have better generalization capabilities, details please refer to the response to the Q2 of Reviewer\#7. 

% This approach differs significantly from DecompDiff, which is a two-stage method and the first stage of DecompDiff involves obtaining a binding prior, specifically several anchor atoms of ligands, to guide the ligand generation process. Furthermore, the ligand priors used in DecompDiff are obtained from the open-source software AlphaSpace. It is important to note that these ligand priors are solely related to the given protein pocket and do not consider the ligand structures. In other words, our method has more generalization capabilities. Furthermore, in comparison to methods that generate molecules based on given templates or priors, such as DecompDiff, our method has the advantage of generating more diverse molecules. This is verified by the diversity metrics presented in \cref{tab:main_tab}.


% \noindent{\textbf{\textcolor{blue}{Q3: Can the authors mention computational complexity details of the proposed method?}}}
\noindent{\textbf{\textcolor{blue}{Q2: Can the authors mention computational complexity details?}}}
% We have conducted a series of experiments to assess the impact of different ratios of nodes in BASE, which factor plays a crucial role in determining the computational complexity and performance of our method, as present in 
% % \cref{rebuttal:select_ratio}. For the complete results, please refer to 
% \cref{appendix:select_ratio} in the Appendix.
% % In practice, we set the the selection ratio to 0.5 from the consideration of the trade-off between performance and efficiency. \zhilin{conclusion}
% We can observe that when r=0.1, our method does not significantly increase the computational cost compared to the baseline model. However, it still achieves a significant improvement in performance. On the other hand, when the r=0.5, the computational complexity of our method is comparable to that of DecompDiff. However, our method outperforms DecompDiff by a significant margin in terms of performance.
% Please refer to \textbf{the Appendix} and \textbf{the response to the Q1 of Reviewer\#7}.
We have conducted a series of experiments to assess the impact of selection ratios in BASE, which factor plays a crucial role in determining the computational complexity and performance of our method, as present in \textbf{Table 5 in the Appendix}.
Please also kindly refer to \textbf{the response to the Q1 of Reviewer\#7} for the detailed explanations.
% \textbf{In conclusion, even simply introducing a little computational complexity ($r$=0.1) can bring a significant improvement in the performance.}

\begin{table}[hp]
    \centering
    \vspace{-2.7mm}
    \begin{adjustbox}{width=0.32\textwidth}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|cc|cc|cc|cc|c}
    \hline
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Vina Score ($\downarrow$)} & \multicolumn{2}{c|}{Vina Min ($\downarrow$)} & \multicolumn{2}{c|}{QED ($\uparrow$)}  & \multicolumn{2}{c|}{Diversity ($\uparrow$)} & Inference Time ($\downarrow$) \\
     & Avg. & Med. & Avg. & Med. & Avg. & Med. & Avg. & Med. & (100 molecules) \\
    \hline
    baseline     & -5.04 & -5.75 & -6.38 & -6.52 & 0.46 & 0.46 & 0.71 & 0.69 & \textbf{1729} s  \\

    r=0.1   & -5.61 & -6.58 & -7.00 & -7.12 & 0.50 & 0.51 & \underline{0.74} & \underline{0.73} & 2060 s \\

    r=0.3   & -5.64 & \underline{-6.64} & \underline{-7.11} & \underline{-7.22} & \textbf{0.52} & \textbf{0.53} & \underline{0.74} & \textbf{0.74} & 2851 s \\

    r=0.5   & \textbf{-5.92} & \textbf{-6.81} & \textbf{-7.29} & \textbf{-7.34} & \underline{0.51} & \underline{0.52} & \textbf{0.75} & \textbf{0.74} & 3372 s \\

    \hline

    TargetDiff & -5.47 & -6.30 & -6.64 & -6.83 & 0.48 & 0.48 & 0.72 & 0.71 & \underline{1987} s  \\

    DecompDiff & \underline{-5.67} & -6.04 & -7.04 & -6.91 & 0.45 & 0.43 & 0.68 & 0.68 & 3218 s  \\

    % \hline

    % Exp5 \\
    % Exp6 \\
    
    \hline
    \end{tabular}
    \renewcommand{\arraystretch}{1}
    \end{adjustbox}
    \vspace{-2mm}
    \caption{Effect of subcomplex selection ratios $r$ in BASE.
    }
    \vspace{-4.5mm}
    \label{rebuttal:select_ratio}
\end{table}


\noindent\textbf{\textcolor{magenta}{--------------------- Response to Reviewer \#7 ------------------}}
% We thank the reviewer for the valuable feedback. Please see below for our responses to the comments. 

% \noindent{\textbf{\textcolor{blue}{Q1: Comparison with existing methods does not seem to be fair in terms of model complexity. Is the time complexity overhead of BindDM worth it while also considering the accompanying model complexity?}}}
% \noindent{\textbf{\textcolor{blue}{Q1: Is the time complexity overhead of BindDM worth it while also considering the accompanying model complexity?}}}
\noindent{\textbf{\textcolor{blue}{Q1: Is the time complexity overhead of BindDM worth it? Is there a fairness issue when it comes to the comparison with existing methods?}}}
% We have conducted a series of experiments to assess the impact of different ratios of nodes in BASE, which factor plays a crucial role in determining the computational complexity and performance of our method, as present in \textbf{\cref{rebuttal:select_ratio}} (complete results are in \textbf{\cref{appendix:select_ratio} of the Appendix}).
The selection ratio in BASE plays a crucial role in determining the model complexity and performance of our method, as presented in \textbf{\cref{rebuttal:select_ratio}} (complete results are in \textbf{\cref{appendix:select_ratio} of the Appendix}).

We can observe that (1) when the ratio \textbf{r=0.1}, our method adds \textbf{almost no computational complexity compared to TargetDiff}. And it still \textbf{achieves a significant improvement in performance}, which is comparable to DecompDiff and outperforms TargetDiff.
% On the other hand, \textbf{when r=0.5, the computational complexity of our method becomes similar to that of DecompDiff. However, our method outperforms DecompDiff by a significant margin in terms of performance}.
% (2) when \textbf{r=0.5}, our method has \textbf{similar computational complexity with DecompDiff} (the consumed time of using external software in DecompDiff is eliminated), while our method \textbf{outperforms DecompDiff by a significant margin in terms of performance}. 
(2) when \textbf{r=0.5} (\textbf{r=0.3}), our method has \textbf{similar computational complexity with (less then) DecompDiff}, while our method \textbf{outperforms DecompDiff by a significant margin in terms of performance}. 
% And DecompDiff requires \textbf{additional software} to provide anchor atoms as templates for the molecular generation.
% And we have ignored the time consume of DecompDiff in utilizing \textbf{additional software} to obtain anchor atoms as templates for the generation.
% And we have \textbf{ignored} the consumed time of utilizing \textbf{external software} to obtain template atoms in DecompDiff.
% And we \textbf{do not} take into account the process of using external softwares to obtain templates atoms in DecompDiff.% when comparing complexity
% And we have \textbf{eliminated the time-consuming step of using external software} in \textbf{DecompDiff} when we calculate the complexity.
Furthermore, the consumed time of \textbf{using external software} in \textbf{DecompDiff} is \textbf{eliminated} when we calculate its complexity.

% Furthermore, it is worth noting that DecompDiff is a two-stage method, which \textbf{relies on an open-source software}, AlphaSpace, to obtain the anchors of generated ligands as \textbf{templates}. This not only reduces the generalization capability (for example, poor diversity and chemical properties as present in \textbf{\cref{tab:main_tab}}), but also adds complexity to the pipeline. In contrast, our method is an end-to-end method does not rely on any external templates, making it more flexible and adaptable in generating diverse and high-quality molecular ligands.
Moreover, we conducted an experiment where the subcomplexes were \textbf{randomly extracted}, as presented in \textbf{Exp1 of \cref{tab:abla_component}}. It indicates that \textbf{simply increasing the model complexity does not necessarily lead to improvements in performance}.
Finally we would like to clarify that the reported inference time refers to the time taken to \textbf{generate a batch of 100 molecules, rather than a single molecule}.

% \textbf{In conclusion, we believe there is no fairness issues in comparing our method with existing approaches, since even simply introducing a little computational and model complexity (r=0.1) can bring a significant improvement.}
In conclusion, we believe there is \textbf{no fairness issues} in comparing our method with existing approaches, since even \textbf{simply introducing a little computational and model complexity (r=0.1) can bring a significant improvement.}

% \noindent{\textbf{\textcolor{blue}{Q3: Boarder Contributions?}}} 
\noindent{\textbf{\textcolor{blue}{Q2: What does the proposed model offer that can benefit the broader AI community?}}} 
% (1) SBDD is an important task in AI for science (AI4S), have raised much attentions in AI community. (2) Our method bridging the gap between the generation tasks and the binding site prediction tasks, can be extended to other tasks in AI4S easily. (3) As stated in the motivation of our method, our approach has the capability to adaptively mine task-related information from redundant graph networks and utilize it to serve the task at hand. This flexibility allows our method to be extended to various tasks related to graphs, including representation learning, key point detection, and more.
(1) SBDD is indeed an important task in the field of AI for science (AI4S) and has garnered significant attention within the AI community. 
% (2) Our method, which \textbf{bridges the gap} between protein-specific molecule generation tasks and binding site prediction tasks, can be easily extended to other tasks within the AI4S domain, like docking pose prediction, etc. 
(2) Our method, which \textbf{connects protein-specific molecule generation tasks and binding site prediction tasks}, can be \textbf{easily extended} to other tasks within the AI4S domain, like docking pose prediction, etc. 
% (3) As stated in the motivation of our method, the ability to adaptively mine task-related clues from redundant information is a key aspect of our approach. This adaptability enables our \method to tackle a wide range of tasks within the AI community, like key point detection, graph representation learning, etc.
(3) As stated in the motivation, the ability to \textbf{adaptively mine task-related clues from redundant information} is a key aspect of our approach. 
It enables our method to be applied in generic graph neural networks to tackle a wide range of tasks within the AI community, like keypoint detection, representation learning, and more.
% It enables our method to tackle a wide range of tasks within the AI community, like key point detection, graph representation learning, etc.

% \noindent{\textbf{\textcolor{blue}{Q2: What are the main differences with the approaches proposed in (Guan et al. 2023a and b) from the view of the scientific gap?}}} 
\noindent{\textbf{\textcolor{blue}{Q3: What are the main differences with the approaches proposed in (Guan et al. 2023a and b)?}}} 
% Both TargetDiff and we proposed \method are \textbf{single-stage} methods generating molecules \textbf{from scratch}. And TargetDiff is our baseline model which treats all the atoms in the pocket equally without considering the information redundancy. 
% The motivation behind our approach is to adaptively exploit essential binding-related subcomplexes from the original complex during the iterative molecule generation process. 
% \textbf{The motivation behind our approach is to adaptively exploit essential binding-related subcomplexes from the original complex during the iterative molecule generation process}. This is designed for enhancing the generation process, as complete complexes often contain a large number of atoms and redundant information is not related to the binding.
% It results in poor generation diversity and chemical properties (like QED), as shown in \textbf{\cref{tab:main_tab}}.
% TargetDiff is our baseline model which treats all the atoms in the pocket equally without considering the information redundancy. 
% \textbf{The motivation behind our approach is to adaptively exploit essential binding-related subcomplexes from the original complex which contains a large number of atoms and redundant binding-unrelated information, during the iterative molecule generation process}.
% Our experiments presented \textbf{\cref{tab:abla_component} (Exp0 and Exp1)} and \textbf{\cref{fig:subcomp_acc}} verified that our method is capable of \textbf{mining some binding-related information} from the original complex.
% Moreover, as present in \textbf{\cref{rebuttal:select_ratio}}, our method only need to introduce of \textbf{small computation burdens (set r=0.1) can achieve significant improvement compared to the TargetDiff}.
% And DecompDiff is a \textbf{two-stage} method and \textbf{totally different} with ours. Specifically, it \textbf{relies on an open-source software, AlphaSpace}, to obtain anchors atoms of generated ligands as \textbf{templates} for the subsequent generation process, which not only \textbf{increases the complexity} of the framework but also \textbf{reduces the generalization ability} of the model, as present in Diversity and QED metrics of \textbf{\cref{tab:main_tab}}. 
% In contrast, TargetDiff and our \method are \textbf{single-stage} method and generate molecules \textbf{from scratch}.
% TargetDiff is our baseline model which generates molecules conditioned on the orginal complex. And DecompDiff is a two-stage method try to introduce pocket prior (i.e. some template atoms of molecules) by using open-source softwares for subsequent generation process. The motivation behind our approach is to adaptively exploit essential binding-related subcomplexes from the original complex which contains a large number of atoms and redundant binding-unrelated information, during the iterative molecule generation process. And our method is a single-stage method, does not rely on any external software and generates molecules from scratch. 
% Extensive experiments results presented \textbf{\cref{tab:abla_component} (Exp0 and Exp1)} and \textbf{\cref{fig:subcomp_acc}} indicates that our method is capable of \textbf{mining some binding-related information} from the original complex. Moreover, as present in \textbf{\cref{rebuttal:select_ratio}}, our method only need to introduce of \textbf{small computation burdens (set r=0.1) can achieve significant improvement compared to the baseline model}.
% TargetDiff, our baseline model, treats all atoms in the pocket \textbf{equally}, \textbf{without explicitly focusing on important information}.
The differences between TargetDiff and our method is that, TargetDiff treats all atoms in the complex \textbf{equally}, \textbf{without explicitly} focusing on binding-related clues from the redundant information.
% TargetDiff is our baseline model, and the main difference with our method is that TargetDiff treats all the atoms in the pocket \textbf{equally}, \textbf{without} considering the \textbf{information redundancy}. 
While our method aims at \textbf{adatively} exploiting the \textbf{essential binding-related substructures} in the original complex, 
% and then uses these essential binding clues for enhancing the generation. 
and then enhance the generation with these binding clues. 

% In conclusion, compare to DecompDiff, our \method \textbf{reduces the complexity} of the framework while \textbf{increasing the generalization ability} of the model (higher diversity in \cref{tab:main_tab}).
% The main differences between our method and DecompDiff are: (1) DecompDiff is a \textbf{two-stage} method, which uses an \textbf{open-source software} to obtain \textbf{several template atoms} of molecules as binding priors for the subsequent generation process. In contrast, our BindDM is a \textbf{single-stage} method and generates molecules \textbf{from scratch}, \textbf{without} introducing any \textbf{external knowledge}. (2) The template atoms, i.e. binding priors, utilized in DecompDiff are \textbf{molecule-agnostic}. On the contrary, our method is able to \textbf{adaptively} mine binding-related subcomplexes by considering the \textbf{interaction between given proteins and molecules during the generation process}. 
% Compared with DecompDiff, our method has a \textbf{simpler framework} and \textbf{better generalization ability} (higher diversity in \cref{tab:main_tab}).

% The main differences between our method and DecompDiff are: (1) DecompDiff is a \textbf{two-stage} method, which uses an \textbf{open-source software} to obtain \textbf{several template atoms} of molecules as \textbf{binding priors} for the subsequent generation process. In contrast, our BindDM is a \textbf{single-stage} method and generates molecules \textbf{from scratch}. It \textbf{adaptively} mines binding-related subcomplexes from the original complex \textbf{without} introducing any \textbf{external knowledge} for enhancing generation process. (2) The binding priors utilized in DecompDiff are \textbf{molecule-agnostic} and only related to proteins, ignoring that different molecules may suggest different binding sites. On the contrary, the binding-related subcomplexes in our method are extracted by considering the \textbf{interaction between given proteins and molecules during the generation process}. 

The main differences between our method and DecompDiff are: (1) DecompDiff is a \textbf{two-stage} method, which uses an \textbf{open-source software} to obtain \textbf{several template atoms} of molecules as \textbf{binding priors} for the subsequent generation process. In contrast, our \method is a \textbf{single-stage} method and generates molecules \textbf{from scratch}. It \textbf{adaptively} mines \textbf{binding-related subcomplexes} from the original complex \textbf{without} introducing any \textbf{external knowledge} for enhancing generation process. (2) The \textbf{binding priors} utilized in DecompDiff are \textbf{solely related to proteins}, ignoring different molecules suggest different binding sites. While, \textbf{binding-related clues} in our method are extracted by fully considering the \textbf{interaction between given proteins and molecules during the generation process}. 

\noindent\textbf{\textcolor{magenta}{--------------------- Response to Reviewer \#8 ------------------}}
% We thank the reviewer for the valuable feedback. Please see below for our responses to the comments. 

% \noindent{\textbf{\textcolor{blue}{Q1: Once the model learns a relevant substructure why include any information beyond the substructure?  Why does the rest of the global structure matter? It would be interesting if the model could identify the substructure then once it is confident discard the rest of the structure.}}}
% \noindent{\textbf{\textcolor{blue}{Q1: Once the model learns a relevant substructure why include any information beyond the substructure?  Why does the rest of the global structure matter?}}}
\noindent{\textbf{\textcolor{blue}{Q1: Once the model learns a relevant substructure why include any information beyond the substructure?}}}
The information included for two reasons: 
% (1) our method \textbf{cannot guarantee} that extracted substructures are completely binding-related and all binding-related substructures can be extracted. This is evident from \textbf{\cref{fig:subcomp_acc}}, where the binding prediction accuracy is not significantly high. Thus, solely relying on extracted substructures is \textbf{insufficient} for the molecule generation, and we need global structures for providing \textbf{global geometric and chemical constraints}. To validate this, we conducted an experiment \textbf{Exp5}, where only substructures of the first layer were used for subsequent generation. The results presented in \textbf{\cref{rebuttal:substructures}} demonstrate that \textbf{discarding} the information beyond substructures \textbf{leads to poor performance};
% (2) Our proposed model performs a hierarchical extraction process where a \textbf{different} substructure is extracted from the original complex at each layer. We believe this allows the model to capture \textbf{richer binding-related substructures}. To investigate this, we conducted an experiment \textbf{Exp6} where we \textbf{fixed} substructures of each layer. The results presented in \textbf{\cref{rebuttal:substructures}} indicate that this approach only led to a \textbf{slight improvement} compared to the baseline.
% And we appreciate the valuable suggestions provided by the reviewer which inspire us to think about whether we can improve the binding metrics of protein-specific molecular generation from the perspective of improving the correlation between extracted substructures and real binding sites. 
% (1) The complete proteins are given conditions, we need complete structures as \textbf{global geometric constraints} to prevent generated 3D molecules from having \textbf{geometric conflicts} with the atoms beyond substructures in proteins. 
% % (The \textit{geometric conflicts} means that the generated molecules \textbf{penetrate} the inner space of protein, which is impossible in the real world).
% Geometric conflicts refer to the situation where the generated molecules \textbf{penetrate} the inner space of proteins, which is \textbf{impossible} in the real world.
% Geometric conflicts are defined as that the generated molecules intrude into the inner space of proteins, which is deemed unattainable in real-world conditions.
% To validate this, we conducted \textbf{Exp5}, where only substructures of the first layer were used for subsequent generation. The results presented in \textbf{\cref{rebuttal:substructures}} demonstrate that \textbf{discarding} the information beyond substructures \textbf{leads to geometric conflicts} (positive Vina scores);
% (1) The complete protein is the given condition, the atoms beyond the substructure may not be related to binding but is \textbf{still a part of the protein}. And we need complete structures as \textbf{global geometric constraints} to prevent generated 3D molecules from \textbf{intruding into the inner space of proteins} (spatial conflicts), which is deemed \textbf{unattainable} in real-world conditions.
(1) The complete protein is the given condition, the atoms beyond the substructure may not be related to binding but is \textbf{still a part of the protein}. And we need complete structures as \textbf{global geometric constraints} to prevent generated 3D molecules from \textbf{intruding into the inner space of proteins}, which is deemed \textbf{unattainable} in real-world conditions.
To validate this, we only use the substructure of the first layer for subsequent generation. The result presented by \textbf{Exp5} in \textbf{\cref{rebuttal:substructures}} indicates that \textbf{discarding} the information beyond substructures leads to \textbf{spatial conflicts} between generated molecules and proteins (positive Vina scores);
(2) Our model performs a hierarchical extraction process where a \textbf{different} substructure is extracted from the original complex at each layer. We believe this allows the model to capture \textbf{richer binding-related substructures}. To investigate this, we fixed substructures of each layer as the substructure of the first layer. And the result presented by \textbf{Exp6} in \textbf{\cref{rebuttal:substructures}} indicates that it brings only \textbf{minor improvements} compared to the baseline.
% And we appreciate the valuable suggestions provided by the reviewer which inspire us to think about whether we can improve the binding metrics of protein-specific molecular generation from the perspective of improving the correlation between extracted substructures and real binding sites. 

% We will take these into consideration in our future work.
% We will take it in our future work.
\begin{table}[hp]
    \centering
    \vspace{-4mm}
    \begin{adjustbox}{width=0.2\textwidth}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|cc|cc|cc}
    \hline
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Vina Score ($\downarrow$)} & \multicolumn{2}{c|}{Vina Min ($\downarrow$)} & \multicolumn{2}{c}{QED ($\uparrow$)}  \\
     & Avg. & Med. & Avg. & Med. & Avg. & Med. \\
    \hline
    baseline     & -5.04 & -5.75 & -6.38 & -6.52 & 0.46 & 0.46  \\

    Exp5   & 11.99 & 3.93 & -0.65 & -4.28 & 0.48 & 0.49  \\

    Exp6   & \underline{-5.48} & \underline{-6.22} & \underline{-6.57} & \underline{-6.70}  & \underline{0.48} & \underline{0.47}  \\

    \method   & \textbf{-5.92} & \textbf{-6.81} & \textbf{-7.29} & \textbf{-7.34} & \textbf{0.51} & \textbf{0.52} \\
    
    \hline
    \end{tabular}
    \renewcommand{\arraystretch}{1}
    \end{adjustbox}
    \vspace{-2mm}
    \caption{Effect of the information beyond the substructures.
    }
    \vspace{-2mm}
    \label{rebuttal:substructures}
\end{table}
